Adaptive Semi-Supervised Segmentation of Brain Vessels with Ambiguous Labels

Accurate segmentation of brain vessels is crucial for cerebrovascular disease diagnosis and treatment. However, existing methods face challenges in capturing small vessels and handling datasets that are partially or ambiguously annotated. In this paper, we propose an adaptive semi-supervised approach to address these challenges. Our approach incorporates innovative techniques including progressive semi-supervised learning, adaptative training strategy, and boundary enhancement. Experimental results on 3DRA datasets demonstrate the superiority of our method in terms of mesh-based segmentation metrics. By leveraging the partially and ambiguously labeled data, which only annotates the main vessels, our method achieves impressive segmentation performance on mislabeled fine vessels, showcasing its potential for clinical applications.

==> reference.tex <==
% \References

\begin{document}

\section*{References}

\begin{thebibliography}{00}

\bibitem{bb7}{
Isensee F, Jaeger P F, Kohl S A A, et al. nnU-Net: a self-configuring method for deep learning-based biomedical image segmentation[J]. Nature methods, 2021, 18(2): 203-211.}

\bibitem{bb1}{Orlov MV, Hoffmeister P, Chaudhry GM, et al. Three dimensional rotational angiography of the left atrium and esophagus–A virtual computed tomography scan in the electrophysiology lab Heart Rhythm 2007;4:37–43.}

\bibitem{bb2}{Ector J, De Buck S, Nuyens D, et al. Adenosine-induced ventricular asystole or rapid ventricular pacing to enhance three-dimensional rotational imaging during cardiac ablation procedures. Europace 2009;11:751–62.}

\bibitem{bb3}{De Potter T J R, Bardhaj G, Viggiano A, et al. Three-dimensional rotational angiography as a periprocedural imaging tool in atrial fibrillation ablation[J]. Arrhythmia and electrophysiology review, 2014, 3(3): 173.}

\bibitem{bb4}{Timmins K M, van der Schaaf I C, Bennink E, et al. Comparing methods of detecting and segmenting unruptured intracranial aneurysms on TOF-MRAS: The ADAM Challenge[J]. NeuroImage, 2021: 118216.}

\bibitem{bb5}{Hennemuth A. Cerebral Aneurysm Detection: First Challenge, CADA 2020, Held in Conjunction with MICCAI 2020, Lima, Peru, October 8, 2020, Proceedings[M]. Springer Nature, 2021.}

\bibitem{bb6}{
Alpers B J, Berry R G, Paddison R M. Anatomical studies of the circle of Willis in normal brain[J]. AMA Archives of Neurology \& Psychiatry, 1959, 81(4): 409-418.}

\bibitem{b02}{
Ma J, Nie Z. Exploring large context for cerebral aneurysm segmentation[C]//International workshop on Cerebral Aneurysm Detection. Springer, Cham, 2020: 68-72.}

\bibitem{b03}{
Yan Z, Yang X, Cheng K T. A three-stage deep learning model for accurate retinal vessel segmentation[J]. IEEE journal of Biomedical and Health Informatics, 2018, 23(4): 1427-1436.}

\bibitem{b01}{
Livne M, Rieger J, Aydin O U, et al. A U-Net deep learning framework for high performance vessel segmentation in patients with cerebrovascular disease[J]. Frontiers in neuroscience, 2019, 13: 97.}

\bibitem{b04}{
Mishra S, Chen D Z, Hu X S. A data-aware deep supervised method for retinal vessel segmentation[C]//2020 IEEE 17th International Symposium on Biomedical Imaging (ISBI). IEEE, 2020: 1254-1257.}

\bibitem{gg1}{
Hilbert A, Madai V I, Akay E M, et al. BRAVE-NET: fully automated arterial brain vessel segmentation in patients with cerebrovascular disease[J]. Frontiers in artificial intelligence, 2020: 78.}

\bibitem{gg5}{
Guo C, Szemenyei M, Yi Y, et al. Sa-unet: Spatial attention u-net for retinal vessel segmentation[C]//2020 25th International Conference on Pattern Recognition (ICPR). IEEE, 2021: 1236-1242.}

\bibitem{a01}{
Shahzad R, Pennig L, Goertz L, et al. Fully automated detection and segmentation of intracranial aneurysms in subarachnoid hemorrhage on CTA using deep learning[J]. Scientific Reports, 2020, 10(1): 1-12.}

\bibitem{a02}{
Kamnitsas K, Ferrante E, Parisot S, et al. DeepMedic for brain tumor segmentation[C]//International workshop on Brainlesion: Glioma, multiple sclerosis, stroke and traumatic brain injuries. Springer, Cham, 2016: 138-149.}

\bibitem{gg2}{
Dengler N F, Madai V I, Wuerfel J, et al. Moyamoya vessel pathology imaged by ultra–high-field magnetic resonance imaging at 7.0 T[J]. Journal of Stroke and Cerebrovascular Diseases, 2016, 25(6): 1544-1551.}

\bibitem{hh1}{
Wang Q, Wang W, Fei Z, et al. Simulation of blood flow in intracranial ICA-PComA aneurysm via computational fluid dymamics modeling[J]. Journal of hydrodynamics, 2009, 21(5): 583-590.}

\bibitem{b05}{
Chen H, Qi X J, Cheng J Z, et al. Deep contextual networks for neuronal structure segmentation[C]//Thirtieth AAAI conference on artificial intelligence. 2016.}

\bibitem{b06}{
Patel T R, Paliwal N, Jaiswal P, et al. Multi-resolution CNN for brain vessel segmentation from cerebrovascular images of intracranial aneurysm: a comparison of U-Net and DeepMedic[C]//Medical Imaging 2020: Computer-Aided Diagnosis. International Society for Optics and Photonics, 2020, 11314: 113142W.}

\bibitem{UNet}{
Ronneberger O, Fischer P, Brox T. U-Net: Convolutional networks for biomedical image segmentation[C]//International Conference on Medical image computing and computer-assisted intervention. Springer, Cham, 2015: 234-241.}

\bibitem{U-Net++}{
Zhou Z, Siddiquee M M R, Tajbakhsh N, et al. UNet++: Redesigning skip connections to exploit multiscale features in image segmentation[J]. IEEE transactions on medical imaging, 2019, 39(6): 1856-1867.}

\bibitem{Dualattention}{
Fu J, Liu J, Tian H, et al. Dual attention network for scene segmentation[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2019: 3146-3154.}

\bibitem{Deepvesselnet}{
Tetteh G, Efremov V, Forkert N D, et al. Deepvesselnet: Vessel segmentation, centerline prediction, and bifurcation detection in 3-d angiographic volumes[J]. Frontiers in Neuroscience, 2020, 14: 1285.}

\bibitem{deepblock}{
Sanchesa P, Meyer C, Vigon V, et al. Cerebrovascular network segmentation of MRA images with deep learning[C]//2019 IEEE 16th International Symposium on Biomedical Imaging (ISBI 2019). IEEE, 2019: 768-771.}

\bibitem{Inception-v4}{
Szegedy C, Ioffe S, Vanhoucke V, et al. Inception-v4, inception-resnet and the impact of residual connections on learning[C]//Thirty-first AAAI conference on artificial intelligence. 2017.}

\bibitem{aneurIST}{
Benkner S, Arbona A, Berti G, et al. @ neurIST: infrastructure for advanced disease management through integration of heterogeneous data, computing, and complex processing services[J]. IEEE Transactions on Information Technology in Biomedicine, 2010, 14(6): 1365-1377.}

\bibitem{cada}{
Ivantsits M, Goubergrits L, Kuhnigk J M, et al. Cerebral Aneurysm Detection and Analysis Challenge 2020 (CADA)[C]//International workshop on Cerebral Aneurysm Detection. Springer, Cham, 2020: 3-17.}

\bibitem{bbb0}{
Dewitte K, Fierens C, Stockl D, et al. Application of the Bland–Altman plot for interpretation of method-comparison studies: a critical investigation of its practice[J]. Clinical chemistry, 2002, 48(5): 799-801.}

\bibitem{bbb1}{
Bland J M, Altman D G. Measuring agreement in method comparison studies[J]. Statistical methods in medical research, 1999, 8(2): 135-160.}

\bibitem{bbb2}{
Bland J M, Altman D G. Statistical methods for assessing agreement between two methods of clinical measurement[J]. The lancet, 1986, 327(8476): 307-310.}

\bibitem{bbb3}{
Weng Y, Zhou T, Li Y, et al. Nas-UNet: Neural architecture search for medical image segmentation[J]. IEEE Access, 2019, 7: 44247-44257.}

\bibitem{bbbb1}{
Kalra M K, Dang P, Singh S, et al. In-plane shielding for CT: effect of off-centering, automatic exposure control and shield-to-surface distance[J]. Korean Journal of Radiology, 2009, 10(2): 156-163.}

\bibitem{bbbb2}{
Kingma D P, Ba J. Adam: A method for stochastic optimization[J]. arXiv preprint arXiv:1412.6980, 2014.}

\bibitem{bbbb3}{
Jadon S. A survey of loss functions for semantic segmentation[C]//2020 IEEE Conference on Computational Intelligence in Bioinformatics and Computational Biology (CIBCB). IEEE, 2020: 1-7.}

\bibitem{bbbb4}{
Li R, Li M, Li J, et al. Connection sensitive attention u-net for accurate retinal vessel segmentation[J]. arXiv preprint arXiv:1903.05558, 2019.}

\bibitem{bbbb5}{
Chen L C, Yang Y, Wang J, et al. Attention to scale: Scale-aware semantic image segmentation[C]//Proceedings of the IEEE conference on computer vision and pattern recognition. 2016: 3640-3649.}

\bibitem{bbbb6}{
Huang Z, Wang X, Huang L, et al. Ccnet: Criss-cross attention for semantic segmentation[C]//Proceedings of the IEEE/CVF International Conference on Computer Vision. 2019: 603-612.}

\bibitem{bbbb7}{
Li H, Xiong P, An J, et al. Pyramid attention network for semantic segmentation[J]. arXiv preprint arXiv:1805.10180, 2018.}

\bibitem{bbbb8}{
Taha A A, Hanbury A. Metrics for evaluating 3D medical image segmentation: analysis, selection, and tool[J]. BMC medical imaging, 2015, 15(1): 1-28.}

\bibitem{cc1}{
Kolesnikov A, Dosovitskiy A, Weissenborn D, et al. An image is worth 16x16 words: Transformers for image recognition at scale[J]. 2021.}

\bibitem{dd1}{
Sugahara T, Korogi Y, Nakashima K, et al. Comparison of 2D and 3D digital subtraction angiography in evaluation of intracranial aneurysms[J]. American Journal of Neuroradiology, 2002, 23(9): 1545-1552.}

\bibitem{dd2}{
Anxionnat R, Bracard S, Ducrocq X, et al. Intracranial aneurysms: clinical value of 3D digital subtraction angiography in the therapeutic decision and endovascular treatment[J]. Radiology, 2001, 218(3): 799-808.}

\bibitem{dd3}{
White P M, Wardlaw J M, Easton V. Can noninvasive imaging accurately depict intracranial aneurysms? A systematic review[J]. Radiology, 2000, 217(2): 361-370.}

\bibitem{dd4}{
van Rooij W J, Sprengers M E, de Gast A N, et al. 3D rotational angiography: the new gold standard in the detection of additional intracranial aneurysms[J]. American Journal of Neuroradiology, 2008, 29(5): 976-979.}

\bibitem{dd5}{
Tanoue S, Kiyosue H, Kenai H, et al. Three-dimensional reconstructed images after rotational angiography in the evaluation of intracranial aneurysms: surgical correlation[J]. Neurosurgery, 2000, 47(4): 866-871.}

\bibitem{ee1}{
Moccia S, De Momi E, El Hadji S, et al. Blood vessel segmentation algorithms—review of methods, datasets and evaluation metrics[J]. Computer methods and programs in biomedicine, 2018, 158: 71-91.}

\bibitem{ee2}{
Firouzian A, Manniesing R, Flach Z H, et al. Intracranial aneurysm segmentation in 3D CT angiography: Method and quantitative validation with and without prior noise filtering[J]. European journal of radiology, 2011, 79(2): 299-304.}

\bibitem{ee3}{
Taher F, Soliman A, Kandil H, et al. Accurate segmentation of cerebrovasculature from TOF-MRA images using appearance descriptors[J]. IEEE Access, 2020, 8: 96139-96149.}

\bibitem{ee4}{
Russ M, O'Hara R, Nagesh S V S, et al. Treatment planning for image-guided neuro-vascular interventions using patient-specific 3D printed phantoms[C]//Medical Imaging 2015: Biomedical Applications in Molecular, Structural, and Functional Imaging. International Society for Optics and Photonics, 2015, 9417: 941726.}

\bibitem{ee5}{
Cebral J R, Mut F, Sforza D, et al. Clinical application of image‐based CFD for cerebral aneurysms[J]. International journal for numerical methods in biomedical engineering, 2011, 27(7): 977-992.}

\bibitem{ee6}{
Chalouhi N, Hoh B L, Hasan D. Review of cerebral aneurysm formation, growth, and rupture[J]. Stroke, 2013, 44(12): 3613-3622.}

\bibitem{ee7}{
Sarrami-Foroushani A, Lassila T, MacRaild M, et al. In-silico trial of intracranial flow diverters replicates and expands insights from conventional clinical trials[J]. Nature communications, 2021, 12(1): 1-12.}

\bibitem{ff1}{
Hernandez M, Frangi A F. Non-parametric geodesic active regions: method and evaluation for cerebral aneurysms segmentation in 3DRA and CTA[J]. Medical image analysis, 2007, 11(3): 224-241.}

\bibitem{ff2}{
Bogunović H, Pozo J M, Villa‐Uriol M C, et al. Automated segmentation of cerebral vasculature with aneurysms in 3DRA and TOF‐MRA using geodesic active regions: An evaluation study[J]. Medical physics, 2011, 38(1): 210-222.}

\bibitem{ff3}{
Hernandez M, Frangi A F. Geodesic active regions using non-parametric statistical regional description and their application to aneurysm segmentation from CTA[C]//International Workshop on Medical Imaging and Virtual Reality. Springer, Berlin, Heidelberg, 2004: 94-102.}

\bibitem{COPEN2016117}{
William A. Copen and Michael H. Lev and Otto Rapalino. Handbook of Clinical Neurology. Chapter 6 - Brain perfusion: computed tomography and magnetic resonance techniques. Elsevier. 2016: 117-135.}

\bibitem{fft1988}{
Brigham E O. The fast Fourier transform and its applications[M]. Prentice-Hall, Inc., 1988.}

\bibitem{pcoma1}{
Golshani K, Ferrell A, Zomorodi A, et al. A review of the management of posterior communicating artery aneurysms in the modern era[J]. Surgical neurology international, 2010, 1.]}

\bibitem{gd}{
Sudre CH, Li W, Vercauteren T, Ourselin S, Jorge Cardoso M. Generalised dice overlap as a deep learning loss function for highly unbalanced segmentations. InDeep learning in medical image analysis and multimodal learning for clinical decision support 2017 Sep 14 (pp. 240-248). Springer, Cham.}

\bibitem{dang2022vessel}{
Dang V N, Galati F, Cortese R, et al. Vessel-CAPTCHA: an efficient learning framework for vessel annotation and segmentation[J]. Medical Image Analysis, 2022, 75: 102263.}


\end{thebibliography}

\end{document}
